Effects of Algorithmic Trend Promotion: Evidence from Coordinated Campaigns in Twitter's Trending Topics

In addition to more personalized content feeds, some leading social media platforms give a prominent role to content that is more widely popular. On Twitter, "trending topics" identify popular topics of conversation on the platform, thereby promoting popular content which users might not have otherwise seen through their network. Hence, "trending topics" potentially play important roles in influencing the topics users engage with on a particular day. Using two carefully constructed data sets from India and Turkey, we study the effects of a hashtag appearing on the trending topics page on the number of tweets produced with that hashtag. We specifically aim to answer the question: How many new tweeting using that hashtag appear because a hashtag is labeled as trending? We distinguish the effects of the trending topics page from network exposure and find there is a statistically significant, but modest, return to a hashtag being featured on trending topics. Analysis of the types of users impacted by trending topics shows that the feature helps less popular and new users to discover and spread content outside their network, which they otherwise might not have been able to do.

==> biblio.tex <==
\begin{singlespace}
\bibliographystyle{alpha}
\bibliography{main-no-zotero-sync}
\end{singlespace}


==> old_results.tex <==
\section{dumping yard: old results}


The fact that a political organization was able to place arbitrary political messages on Twitter's front page would be enough to alarm many concerned with social media and election interference. Indeed, many assume that what Twitter promotes as \textit{trending} is important in some way. To assess the effectiveness of these campaigns and therefore craft a proportional response, we must first consider the goal of these campaigns. The stated campaign objective of \textit{trending} is only a means to an end. While we can not know what the organizers of these WhatsApp groups wanted specifically, there are a few reasonable goals for such a campaign:

\begin{itemize}
	\item \textbf{Spread pro-Modi messages to raise support and influence elections.} Political groups want power. These campaigns could have been cost-effective advertising. By elevating their messages to Twitter's Trending Topics page, they hoped to expose moderate voters to pro-Modi messages and win votes. 
	
	\item \textbf{Set the agenda for political discussion on Twitter.} A similar but less ambitious goal to spreading pro-Modi messages is to \textit{set the agenda}. Perhaps convincing people of Modi's agenda or converting voters is too difficult, but by elevating certain hashtags to Trending Topics, they could control \textit{what} is being discussed in a way favorable to the BJP.
	
	\item \textbf{Build comradery among existing Modi base.} One possible motivation behind these campaigns is to foster a sense of comradery among the BJP. This digital canvassing may not have been intended to win over voters, but to cater to the ``sports fandom'' flavor of politics prevalent on social media. Kevin Munger labels it \textit{connective effervescence}: ``the goal is partially to antagonize your opponents and hearten your allies, but more directly, to become part of living mass of people.'' \cite{mungerStreamingChatConnective2021} 
\end{itemize}


\section{Message Persistence} \label{message_persistence}
Did the messages behind the template tweets persist in the discussion within the hashtags they popularized? It may not be relevant that the template tweets were not popular or influential directly so long as they \textit{seeded} the conversations effectively. That other tweets simply used the astroturfed hashtag is some indication of successful agenda setting, but the template hashtags are generally broad, such as simply stating support for Modi or the military. Assuming users aim to tweet within the boundaries set by a hashtag, generic hashtags give users considerable latitude in terms of tweet content. 

Below, I propose a novel approach to evaluating this message persistence through semantic similarity. I attempt to measure the extent to which the tweets using the hashtag are discussing the same points as the original template tweets. I will refer to this as message persistence rather than agenda setting because of the causal connotation of agenda setting. While I will not make causal claims, measuring message persistence in this way can evaluate how consistent the broader conversation was with the initial pro-BJP talking points seeded by the template tweets. Moreover, message persistence can be thought of as a \textit{prerequisite} for agenda setting. Thus, evidence of absence of message persistence is evidence against agenda setting.

\subsection{Methods}
It is helpful to think of message persistence graphically. Consider Figure \ref{fig:semantic_agenda_setting}. Each circle is a tweet. The distances between circles are proportional to semantic similarity. In other words, tweets with similar meaning are close to each other, while tweets about different things are far apart. Consider a campaign that has tweets on three separate topics with four template tweets about each topic. As in Figure \ref{fig:semantic_agenda_setting}, we would observe three clusters of four tweets. How, then, would we detect if other users are discussing these topics? We would see normal tweets cluster around the template tweets. Figure \ref{fig:semantic_agenda_setting} represents a campaign in which there was successful agenda setting on Topic 2, but not on the other topics. After the template tweets, ``normal users'' are discussing similar themes. While we cannot determine that users are posting these tweets \textit{because} of the template tweets, they are nevertheless engaging with the same topics as the template tweets. In other words, it \textit{looks} like agenda setting and indicates the conversation has not drifted beyond the design of the campaign originators.

\begin{figure}[ht]
	\centering
	\begin{subfigure}[b]{.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{twitter/semantic_agenda_setting.png}
		\caption[Semantic Agenda Setting]{Semantic Agenda Setting}
		\label{fig:semantic_agenda_setting}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{twitter/template_penetration_explainer.png}
		\caption[Template Penetration Rate]{Template Penetration Rate}
		\label{fig:tpr_explainer}
	\end{subfigure}
	\caption[Semantic Similarity Overview]{Semantic Similarity Overview}
	\label{fig:semantic_similarity}
\end{figure}

I start by cleaning and processing the tweets to remove links, tags, hashtags, and duplicates. Once I have the raw text of the tweet, I embed each unique tweet as a vector representation using a pre-trained, multi-lingual sBERT model \cite{reimersSentenceBERTSentenceEmbeddings2019}. I fixed the neighborhood size to be equal to the nearest 1\% of all unique hashtag tweets. I removed hashtags with fewer than 3000 unique tweets. 

The statistic I will use to quantify message persistence is Template Penetration Rate (TPR). TPR refers to the proportion of template tweets in a given tweet's neighborhood. Figure \ref{fig:tpr_explainer} communicates this idea visually. It follows that if the resulting conversations were largely about the topics seeded by the template tweets, the template tweets will have a \textit{low} TPR because many of the tweets around it will be normal tweets engaging with similar content. Conversely, a high TPR for a template tweet indicates that there is not much normal conversation around the same subject. For normal tweets, the opposite is the case; a low and high TPR indicate low and high message persistence, respectively. 

I present TPR results normalized by hashtag-wide template frequency. For example, if 90\% of tweets in a given hashtag are templates, then \textit{of course} there will be a high TPR. So, we normalize this by 90\% to get a statistic that is relative to the template/normal split within the hashtag. This normalized TPR statistic is equal to one if the neighborhood composition of template to normal tweets is \textit{identical} to the hashtag-wide composition. 

\subsection{Results}
Figure \ref{fig:template_penetration} depicts the distribution of normalized TPR for template and normal tweets. Each line is a different hashtag, and the opacity is set based on the number of tweets in that hashtag.

Note how clearly we see the difference in distributions. Template tweets mostly have high TPR, meaning their neighbors are mostly template tweets. The small slope at low TPR values indicates that very few template tweets show message persistence. In short, there is significant clustering between the template tweets and normal tweets in the embedded space. Template tweets are similar semantically to other template tweets, while normal tweets are similar semantically to normal tweets. For many of the hashtags, more than 75\% of the normal tweets  do not have a single template tweet in their 1\% neighborhood. This is largely consistent with the conclusions from the previous analysis; just as the template tweets were not retweeted by normal users, the messages in template tweets were not discussed by the normal users either. Overall, there is a lack of interaction between template tweets and the rest of the tweets using the hashtag.

\begin{figure}[ht]
	\centering
	\includegraphics[width=.6\linewidth]{twitter/template_penetration_cdfs_1percent.png}
	\label{fig:template_penetration_1percent}
	\caption[Template Penetration Rates by Tweet Type]{Template Penetration Rates by Tweet Type}
	\label{fig:template_penetration}
\end{figure}

This TPR concept is useful for extracting template tweets that had high message persistence. One such example of a template tweet with a low TPR can be found in Figure \ref{fig:agenda_setting_example}. The hashtag is about expressing pride in Modi. The template tweet talks about Modi's anti-corruption investigations. Many normal tweets appeared later \textit{also} discussing this theme of financial corruption. Again, this does not suggest that the template tweet \textit{caused} these later tweets, but it does suggest high message persistence for this topic. 

\begin{figure}[ht]
	\centering
	\includegraphics[width=.8\linewidth]{twitter/agenda_setting_example.png}
	\caption[Semantic Agenda Setting Example]{Example of an agenda setting template tweet. The template tweet is about corruption and Modi putting a stop to it. The hashtag, which is about expressing pride over Modi, features many other tweets about corruption.}
	\label{fig:agenda_setting_example}
\end{figure}


While this NLP approach makes it difficult to make any causal claims, it does provide some insight into message persistence. If we found high message persistence across the board, we would not be able to attribute it to the template tweets. However, we found low message persistence, which means there could not have been significant agenda setting.



\section{Evaluating Campaign Efficacy} \label{prelim}
In the following chapter, I examine the efficacy of the ``trend attacks'' based on metadata and metrics proposed in previous work. Specifically, I aim to answer the following questions:

\begin{itemize}
	\item How popular were the template tweets? 
	\item Who spreads template tweets? 
	\item How influential are the campaign participants compared to non-participants?
	\item How does exposure to template tweets and normal tweets relate to a user's decision to use a hashtag?
\end{itemize}

\subsection{Data set} 


\subsection{How do Template Tweets Spread Throughout The Network?}
By a first approximation, template tweets are not as successful as normal tweets. Looking at the distribution of retweets by tweet type in Figure \ref{fig:cascade_size_hist}, it's clear that template tweets did not receive as many retweets as normal tweets. No template tweets received more than 150 retweets. The low retweet numbers suggest that the high-degree users of Indian political Twitter did not retweet template tweets to their many followers. If they had, we would expect to see tweets with more than 150 retweets.

\begin{figure}[ht]
	\centering
	\includegraphics[width=.5\linewidth]{twitter/cascade_size_by_tweet_type_hist.png}
	\caption[Cascade Size Histogram by Tweet Type]{Cascade Size Histogram by Tweet Type}
	\label{fig:cascade_size_hist}
\end{figure}

Another relevant question is who is helping to spread the tweets (along with the hashtag) \textit{within} the cascades. The number of total retweets obscures the impacts of the individuals who are actually responsible for propagation within the retweet cascade. Such an example where much of the spread comes from someone other than the original poster can be found in Figure \ref{fig:cascade_example}. For the purposes of this analysis, I rely on the ``last retweeter'' cascade construction method, where ambiguous retweet attributions go to the user's friend who most recently retweeted \cite{goelStructureOnlineDiffusion2012}. I study the implied retweets for each user, or the number of children of each user within a reconstructed retweet cascade. Figure \ref{fig:cascade_propogaters} shows the number of implied retweets by user type for template tweets and all tweets. 


\textbf{Do non-participants spread template tweets?}
From Figure \ref{fig:template_cascade_by_user}, it is clear that non-participants did not help propagate template tweets. In fact, almost all of the people spreading the template tweets via retweet were campaign participants. The same people posting the template tweets are retweeting them. This result suggests weak penetration of the template tweets into the rest of the Twitter network; outside of the insular volunteer network, users did not endorse the template tweets. 

\textbf{Did campaign participants determine popular tweets?}
On the other hand, non-participants were largely responsible for the spread of tweets within the hashtag, and almost solely responsible for the high-impact spreading, as they dominate the right tail of Figure \ref{fig:normal_cascade_by_user}. If campaign participants were playing a large role in the spread of normal tweets, this might indicate maintained campaign control over the hashtag. The absence of campaign participants in the retweet cascades of the most impactful tweets may suggest the general conversation around the hashtag takes on a new meaning beyond what the campaign originators intended. I explore this idea of message persistence in Section \ref{message_persistence}.

\begin{figure}[ht]
	\centering
	\begin{subfigure}[b]{0.48\textwidth}
	\centering
	\includegraphics[width=\linewidth]{twitter/template_tweet_popularity_by_user_type.png}
	\caption[Template Cascade Histogram]{Number of Cascade Descendants by User Type, Template Tweets}
	\label{fig:template_cascade_by_user}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{twitter/normal_tweet_popularity_by_user_type.png}
		\caption[Normal Cascade Histogram]{Number of Cascade Descendants by User Type, All Tweets}
		\label{fig:normal_cascade_by_user}
	\end{subfigure}
	\caption[Cascade Descendants by User Type]{Cascade Descendants by User Type}
	\label{fig:cascade_propogaters}
\end{figure}


\subsection{Exposure Curves}
How does exposure to template and normal tweets drive hashtag engagement? I draw on previous work by Romero et al. and create exposure curves for hashtag engagement  \cite{romeroDifferencesMechanicsInformation2011}. These curves show the empirical cumulative distribution function (ECDF) of the number of exposures to the hashtag \textit{prior} to first hashtag use for each user. Here, exposure is the number of tweets observed  through a user's follower network. Figure \ref{fig:exposure_curves} depicts three ECDFs corresponding to exposure to template tweets, exposure to normal tweets, and exposure to both tweets. 

Figure \ref{fig:exposure_curves} demonstrates that much of hashtag participation is \textit{not} driven by template tweets. The left-most plot, which represents the normal tweet exposure curve,  shows that nearly 45\% of normal tweets received \textit{no} exposure to template tweets. In contrast, only 10\% of users received no exposure to normal tweets before hashtag adoption. Nearly every hashtag user is exposed to the hashtag prior to posting; only 2.5\% of all tweets came without exposure through the follower network.  This low number, in contrast with Romero's finding that 29\% of tweets come from external events, reflects the absence of a large external event \cite{romeroDifferencesMechanicsInformation2011}. 

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{twitter/exposure_curves.png}
	\caption[Exposure Curves]{Distribution of Exposures to Hashtag Prior to First Hashtag Use}
	\label{fig:exposure_curves}
\end{figure}


\subsection{Summary}
Standard approaches to gauging influence indicate that the template tweets were not influential. They did not gain many retweets and they were not embraced by the high degree nodes within Indian political Twitter. In fact, most users that retweeted the template tweets were other participants in the campaign. Moreover, campaign participants did not play much of a role in the spread of popular normal tweets. Finally, exposure to template tweets does not appear to drive the majority of hashtag use. Overall, these findings suggest the campaigns may have had a minimal agenda setting impact.

If template tweets, and by extension campaign originators, were not influential within the hashtags, this may suggest that normal tweets took on a different meaning from that intended by the campaign originators. I explore this topic in the following section.



